Can User-Level Probing Detect and Diagnose Common Home-WLAN Pathologies?

Common WLAN pathologies include low signal-to-noise ratio, congestion, hidden terminals or interference from non-802.11 devices and phenomena. Prior work has focused on the detection and diagnosis of such problems using layer-2 information from 802.11 devices and special-purpose access points and monitors, which may not be generally available. Here, we investigate a userlevel approach: is it possible to detect and diagnose 802.11 pathologies with strictly user-level active probing, without any cooperation from, and without any visibility in, layer-2 devices? In this paper, we present preliminary but promising results indicating that such diagnostics are feasible.

==> Makefile <==
REPORT=paper
LATEX=latex
BIBTEX=bibtex --min-crossrefs=1000
REF1=ref2

TEX = $(wildcard *.tex)
CLS = $(wildcard *.cls)
SRCS = $(TEX)
REFS=$(REF1).bib

all: pdf
#.tex.dvi:
#       $(LATEX) $*.tex

#$(REPORT).dvi: figures $(SRCS) $(CLS) paper.bib
$(REPORT).dvi: $(SRCS) $(CLS) $(REF1).bib
	$(LATEX) $(REPORT)
	$(BIBTEX) $(REPORT)
	perl -pi -e "s/%\s+//" $(REPORT).bbl
	$(LATEX) $(REPORT)
	$(LATEX) $(REPORT)

#$(REPORT).ps: $(REPORT).dvi figures
$(REPORT).ps: $(REPORT).dvi 
	dvips -Pcmz -t letter $(REPORT).dvi -o $(REPORT).ps
#	dvips -Ppdf -G0 -t letter $(REPORT).dvi -o $(REPORT).ps



#not relevant here
#figures:
#	cd figures; make


view: $(REPORT).dvi
	xdvi $(REPORT).dvi

print: $(REPORT).dvi
	dvips $(REPORT).dvi

pdf: $(REPORT).ps
	ps2pdf14 $< $(REPORT).pdf

printer: $(REPORT).ps
	lpr $(REPORT).ps

tidy:
	rm -f *.dvi *.aux *.log *.blg *.bbl

clean:
	rm -f *~ *.dvi *.aux *.log *.blg *.bbl $(REPORT).ps $(REPORT).pdf $(PROPOSAL).ps $(PROPOSAL).pdf $(FIRSTDRAFT).ps $(FIRSTDRAFT).pdf



==> conclusion.tex <==
\section{Conclusion}



==> eval.tex <==
\section{Evaluation - Accuracy}

We show false-detection rates for each of the above pathologies. An
accuracy matrix would be a good illustration:

%
\begin{table*}
\begin{centering}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline 
\multicolumn{8}{|c|}{\textbf{Diagnosis}}\tabularnewline
\hline 
 &  & CC & CT & HT & SNR & non-802.11 & no-diagnosis\tabularnewline
\cline{2-8} 
 & CC &  &  &  &  &  & \tabularnewline
\cline{2-8} 
\textbf{Pathology} & CT &  &  &  &  &  & \tabularnewline
\cline{2-8} 
 & HT &  &  & (fraction of detections) &  &  & \tabularnewline
\cline{2-8} 
 & SNR &  &  &  &  &  & \tabularnewline
\cline{2-8} 
 & non-802.11 &  &  &  &  &  & \tabularnewline
\hline
\end{tabular}
\par\end{centering}

\caption{Detection accuracy matrix.}

\end{table*}




==> objectives.tex <==
\section{Architecture, Probing and Diagnosis Tree}

We consider the following architecture, which is typical for most
home WLANs (see Figure \ref{fig:System-architecture.}). A single
802.11 Access Point (AP) is used to interconnect a number of wireless
devices; we do not make any assumptions about the exact type of the
802.11 devices or AP

Our experiments have been conducted using 802.11g devices. 
The testbed consists of Soekris \texttt{net4826} nodes with
mini-PCI interfaces. The mini-PCI interfaces host either an Atheros
chipset or an Intel 2915ABG chipset, with the madwifi and ipw2200
drivers respectively (on the Linux 2.6.21 kernel). The madwifi driver
allows us to choose between four different rate adaptation modules.
We disable the madwifi features of 802.11g referred to as
{\em fast frames} and {\em bursting} in our experiments\XXX{, since
they are specific to madwifi's \emph{Super-G} implementation}.

We assume that another computer, used as our WLAN-probe measurement
server $S$ is connected to the AP through an Ethernet connection.
This is not difficult in practice given that most APs provide an Ethernet
port, as long as the user has at least two computers at home. 
\XXX{This wired link can be arbitrarily long, as long as the jitter it
introduces is much smaller than 802.11 delays.}
The server $S$ allows us to probe the WLAN channel without requiring
\emph{ping-like} replies from the AP and without distorting the forward-path
measurements with reverse-path responses. The measurements can be
conducted either from $C$ to $S$ or from $S$ to $C$; we focus
on the former. Note that some APs or terminals that are not a part
of our WLAN may be nearby (e.g., from other home networks)
creating hidden terminals and/or interference.

%
\begin{figure}
\begin{centering}
\includegraphics[width=0.4\textwidth]{system}
\par\end{centering}

\caption{System architecture.\label{fig:System-architecture.}}

\end{figure}


\XXX{The probing phase consists of 100 back-to-back UDP packet trains.
These packet trains are sent from the WLAN-probe client $C$ to the
WLAN-probe server $S$. The packets are timestamped at $C$ and $S$
so that we can measure their \emph{relative} One-Way Delay (OWD) variations; the two
hosts do not need to have synchronized clocks, and we compensate for
clock skew \XXX{for each train by subtracting its minimum OWD}. The send/receive timestamps are obtained at user-level.
There is an idle time of a second or more between successive packet
trains. Each train consists of 50 packets of different sizes; the
rationale for variable-size packets will become clear in subsequent
sections. About 10\% of the packets are of the minimum-possible size
(8-bytes for a sequence number and a send-timestamp, together with
the UDP/IP headers) and they are referred to as \emph{tiny-probes}
- they play a special role in transmission rate inference. The size
of the remaining packets is uniform randomly chosen from the set of values
$\{8+200\times k,k=1\dots7\}$ bytes.}

\XXX{Figure \ref{fig:Decision-tree.} shows the WLAN-probe diagnosis tree.
We start by analyzing each packet train separately, and use a novel
dispersion-based method to infer the per-packet layer-2 transmission rate,
when possible (Section \ref{sec:Rate-Inference}). Based on the
inferred rates, we can measure a certain metric, referred to
as \emph{wireless access delay} or simply \emph{access delay}, for
each packet (Section \ref{sec:Access-Delays}). We then examine whether
the access delays increase with the packet size 
(Section \ref{sec:Low-Signal-Strength}).
When this is \emph{not} the case, the WLAN pathology is diagnosed
as congestion. 
On the other hand, when the access delays increase with the
packet size, the observed pathology is due to low SNR or hidden terminals.
We distinguish between these two pathologies based on temporal correlation
properties of packets that either encountered very
large access delays or that were lost at layer-3 (Section
\ref{sec:Hidden-Terminals-and}).}

%
\begin{figure}
\begin{centering}
\includegraphics[width=0.4\textwidth]{flowchart}
\par\end{centering}

\caption{WLAN-probe decision tree.\label{fig:Decision-tree.}}

\end{figure}




